Vision and Control for Grasping Clear Plastic Bags

We develop two novel vision methods for planning effective grasps for clear plastic bags, as well as a control method to enable a Sawyer arm with a parallel gripper to execute the grasps. The first vision method is based on classical image processing and heuristics (e.g., Canny edge detection) to select a grasp target and angle. The second uses a deep-learning model trained on a human-labeled data set to mimic human grasp decisions. A clustering algorithm is used to de-noise the outputs of each vision method. Subsequently, a workspace PD control method is used to execute each grasp. Of the two vision methods, we find the deep-learning based method to be more effective.

==> bib_commands.tex <==
****** Note: this is not a real tex document. I just gave it the extension so that you'd get tex-style syntax highlighting ******

Rather than using the bibitem package, as the IEEE sample does, I recommend using BibTex. Copy the bibliography folder into the folder containing your main document. Before the \begin{document}, you should include

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

At the end of your file, before the \end{document}, you should include

\bibliographystyle{./bibliography/IEEEtran}
\bibliography{./bibliography/IEEEabrv,./bibliography/references}

All your citations should go inside \verb=/bibliography/references.bib=. Remember that you can usually download a BibTex citation for any resource you use from Google Scholar or Arxiv, and just copy it into \verb=references.bib=. 



